Cache Telepathy: Leveraging Shared Resource Attacks to Learn DNN Architectures

Deep Neural Networks (DNNs) are fast becoming ubiquitous for their ability to attain good accuracy in various machine learning tasks. A DNN's architecture (i.e., its hyper-parameters) broadly determines the DNN's accuracy and performance, and is often confidential. Attacking a DNN in the cloud to obtain its architecture can potentially provide major commercial value. Further, attaining a DNN's architecture facilitates other, existing DNN attacks. This paper presents Cache Telepathy: a fast and accurate mechanism to steal a DNN's architecture using the cache side channel. Our attack is based on the insight that DNN inference relies heavily on tiled GEMM (Generalized Matrix Multiply), and that DNN architecture parameters determine the number of GEMM calls and the dimensions of the matrices used in the GEMM functions. Such information can be leaked through the cache side channel. This paper uses Prime+Probe and Flush+Reload to attack VGG and ResNet DNNs running OpenBLAS and Intel MKL libraries. Our attack is effective in helping obtain the architectures by very substantially reducing the search space of target DNN architectures. For example, for VGG using OpenBLAS, it reduces the search space from more than $10^{35}$ architectures to just 16.

==> discussion.tex <==

%We now discuss two avenues of future work.

%\paragraph{Learning additional parameters}
Our attack learns DNN hyper-parameters that are visible at inference time.  
Several training-time parameters (e.g., training batch size, learning rate, which layers use batch normalization~\cite{batchnormalization}) are not visible at inference time.
Nonetheless, there are standard default practices for setting most training parameters (e.g., modern networks apply batch normalization after each convolution~\cite{ResNet}). 
It is also possible to hide several inference-time parameters.
Currently our attack cannot determine (a) exact filter or input dimensions if the filters/inputs are not square, (b) non-unit stride from pooling layers, or (c) which variant of the Relu non-linearity~\cite{ReluVariants} is used.
%For example, our attack learns $R_i^2$ and assumes $R_i$ is a square number (likewise for input dimensions).
%Clearly, we can detect non-square filters but can be left with several possible aspect ratios depending on the factorization of matrix dimensions.
%Lastly, the current attack cannot disambiguate non-unit stride with pooling layers.

\begin{comment}
\paragraph{Attacking GPUs}
%\todo{Not sure how to fit CPU in this pargaraph.}
As stated earlier, our attack works on CPUs, which are popular platforms for DNN inference for their competitive low latency,
while our attack can also be extended to GPUs,
since the GEMM implementation on GPUs is optimized for multi-level caches using similar blocking and buffering strategies.
%Our attack is the stepping stone for future research on DNN attacks, 
%including attacks on GPUs.
%Several insights from our attack can be applied on GPUs.
%GEMMs on GPUs are operated by multiple parallel threads,
In this paper, we have provided a detailed and thorough analysis on
different aspects, optimizations, and implementations of GEMM attacks.
We envision that a successful attack on GPUs need to leverage our analysis and 
follow a similar attack procedure.
The only extra component is an additional attack primitive to handle the noise introduced by parallelism,
%Considering the highly parallelism in GPU setup, we need
which we can leverage recent techniques on GPU covert channel attacks~\cite{gpu_covert}.
%\todo{as stated earlier, cpus are popular platform for inference for its low latency.
%reference MICRO covert channel work on GPUs.}
\end{comment}

%\todo{mention gpp is preferred in dnn inference compared to GPU in introduction.
%And also claim GPP is still dominant for inference. cite a paper about doing
%inference on GPU incurs high latency. GPU does now work well for small batch size, 
%and generally inference uses small batch size.}


\begin{comment}
\paragraph{Learning DNN structure given non-sequential layers.}
Our current attack also assumes layer organization is sequential, and that layer $i$ only routes to layer $i+1$ (e.g., \cite{Alexnet,simonyan2014vgg}).
This is not the case for several proposals~\cite{DenseNets,ResNet,Googlenet}.
Residual learning~\cite{ResNet,DenseNets} - which allows connections to skip layers - is becoming a standard practice.
In that case, an adversary can assume the victim network will have skip connections.
Networks based on repeating a smaller module (e.g., the inception module~\cite{Googlenet}) cannot be fully disambiguated by our current attack.
In this case, the attacker learns a linearized ordering of layers in a module.


1. GoogleNet
2. secure matrix multiplication implementation
3. Unrecoverable parameters, such as batch normalization, stride, training batch size.
\end{comment}

==> motivation.tex <==

\todo{Need a name for our attack. Is there a better one than "model structure extraction attack"?}
\todo{maybe architecture extraction attack?}

Attacks targeting machine learning algorithms have become a serious security threat.
Previous researchers have shown that these attacks are very effective in revealing attributes of private training data.
Claimed as black-box attacks, however, when attacking neural networks,
these attacks all require to know the \textbf{structure of oracle model},
which is generally not public information.
Moreover, there do not exist practical approaches to steal model structures.
In this section, we discuss the motivation to design an effective model structure extraction attack.

\subsection{Importance of obtaining oracle model structure}

Obtaining oracle model structure is an essential prerequisite of multiple types of attacks,
including model extraction attacks, model inversion attacks and membership inference attacks.
Since the attacker is assumed to have no access to neither oracle training nor test data set,
a common step of all these attacks is to retrain a substitute neural network using synthetic data sets.

\todo{need two things from the VGG test: that model extraction accuracy is greatly impacted by parameters and that searching the space is hard.}

\todo{Need to make this paragraph more logical and clear.}
In both membership inference attacks and model inversion attacks, 
the substitute models must be trained in the same way as the oracle model~\cite{shokri2016membership}.
This is because their attacks are based on a very important assumption,
that is, models with the same structure should behave similarly.
For example, membership inference attacks try to analyze how differently oracle model behaves 
on data points within or out of its training data set.
Unable to access the oracle training data set,
the attacker carries out the analysis on multiple substitute models using the same model structure as oracle one.
The analysis results are then applied to the oracle model.
The applicability is mostly determined by how much similar the substitute models are to the oracle model.
Therefore, Obtaining the model structure is an essential step of both attacks.


In model extraction attacks~\cite{tramer2016stealing}, 
the retraining must use the same architecture as oracle network to achieve good fidelity.
To further validate this claim, we show an example of model extraction attack.
We train an oracle network $f$ using training and test data set from Human Activity Recognition database
~\footnote{http://archive.ics.uci.edu/ml/datasets/Human+Activity+Recognition+Using+Smartphones}.
The oracle has 2 fully-connected layers with 1024 neurons in each layer and a softmax layer.
We use $Tanh$ as the activation function.
We then use adaptive retraining techniques~\cite{tramer2016stealing,cohn1994improving,settles2010active}
to train four different substitute networks.
The four networks $\hat{f}\{1-4\}$ have $1$ to $4$ fully-connected layers respectively. 
Their other hyper-parameters are exactly the same as the oracle network.
Note that in a real attack scenario, the attacker has to pick among much more architectures.


\todo{Need to mention the attacker can obtain confidence value.}
The retraining operates for some number of rounds.
In the first round, it queries the oracle on $m$ uniform random points,
and trains a model $\hat{f}_{(1)}$. At the end of each round $r$, it generates new data points around the 
decision boundary of $\hat{f}_{(r)}$ using jacobian augmentation technique~\cite{papernot2016practical},
which are then added to the training set to train $\hat{f}_{(r+1)}$.
The validation set is derived in the same way as training set.
In Table~\ref{tab:motivation}, we show retraining accuracy on
the synthetic validation set and the oracle test data set,
where the latter one is not accessible to the attacker.
The accuracy is obtained after $7$ rounds, using $1500$ initial random points.


\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|c|}
    \hline
    substitute  &  accuracy on                  & accuracy on   \\
      model     &  synthetic validation set     & oracle test set     \\\hline\hline
    $\hat{f}1$  &  98.24\%  &  23.12\%  \\\hline
    $\hat{f}2$  &  98.90\%  &  \textbf{94.25\%}  \\\hline
    $\hat{f}3$  &  99.09\%  &  92.28\%  \\\hline
    $\hat{f}4$  &  99.12\%  &  91.72\%  \\\hline
    \end{tabular}
    \caption{Retraining accuracy of different substitute models.}
    \label{tab:motivation}
\end{table}


\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|c|}
    \hline
    substitute  &  accuracy on                  & accuracy on   \\
      model     &  synthetic validation set     & oracle test set     \\\hline\hline
    $\hat{f}1$  &  28.65\%  &  18.43\%  \\\hline
    $\hat{f}2$  &  97.72\%  &  \textbf{96.87\%}  \\\hline
    $\hat{f}3$  &  90.39\%  &  90.78\%  \\\hline
    $\hat{f}4$  &  92.55\%  &  91.72\%  \\\hline
    \end{tabular}
    \caption{Retraining accuracy of different substitute models. Validation uses a small subset from oracle test set.}
    \label{tab:motivation2}
\end{table}

The goal of retraining is to obtain a substitute model works as similar as the oracle one
on the oracle test set. 
All of $\hat{f}\{1-4\}$ get similar accuracy (around 99\%) on synthetic validation sets.
$\hat{f}1$ performs the worst on oracle test set due to its simple architecture.
$\hat{f}2$, which uses the same architecture as the oracle model,
gets the highest accuracy (more than 95\%).
Even though $\hat{f}3$ and $\hat{f}4$ uses deeper network architecture, which is supposed
to adapt to more complicated decision boundaries, they achieve lower accuracy than $\hat{f}2$.
Moreover, the deeper the network is, the more computation resources it consumes.
Therefore, obtaining the structure of the oracle model is an essential requirement for efficient and high-quality
model extraction attacks.

\subsection{Ineffectiveness of existing model structure extraction approaches}
\todo{Is this subtitle ok? Shokri et al. do not steal the model.}

There is no effective and practical way to steal the structure of a neural network.
To the best of our knowledge, there are only two work discussed how to train a substitute model
using the same architecture as the oracle one.
We found neither of the approaches is effective.


Ateniese et al.~\cite{ateniese2015hacking} assumes the attacker can access to the binary executable
files for the target model, and thus can extract the structure and parameters
of oracle model via static or dynamic binary analysis techniques.
This approach is unlikely to work since model owner generally hosts the model in the cloud,
and does not release the executable files for confidential models.

Instead of stealing the model structure, 
Shokri et al.~\cite{shokri2016membership} shows that, 
if using the same MLaaS platform (e.g. Google Prediction API)
for the same type of machine learning tasks, empirically the same model structure 
will be used by the service provider.
Thus, the attacker can simply use exactly the same service to train substitute model
as was used to train the oracle model.
However, it can only apply to limited platforms, which always use default model structures.
%only works for platforms which do not provide any freedom for users to customize model structure,
It does not work for other MLaaS platforms, which allow users
to customize their own neural networks.
For example, in Microsoft Azure ML, users are allowed to select type of neural networks, 
number of layers and neurons in each layer etc.
Such fine-grained customization can help users to find the best architecture for their machine learning tasks.

Another possible approach to figure out the oracle model structure is brute force search.
An attacker can train multiple candidate models using all possible architectures 
and use the one with highest accuracy as real substitute model.
However, this approach is extremely inefficient and only works if the attacker can obtain a good validation set.
%and consumes too much resources.
In the case that the attacker does not have any knowledge about the distribution of the oracle test set,
it can only evaluate substitute models based on their accuracy on a synthetic validation set with randomly generated data points.
Table~\ref{tab:motivation} shows this approach is ineffective.
The model with the highest validation accuracy
does not have the same structure as the oracle and does not perform well on oracle test set.
\todo{discuss the case that brute force search works, but it is very inefficient.
Space search is not convex??
Takes multiple GPU days, but our attack works for only several minutes.} 



In summary, oracle model structure is an important information for multiple attacks,
while there does not exist an effective approach to steal it.
In this paper, we propose to extract model structure using cache-based side channel attacks.
Our attack results will strengthen multiple other attacks,
and thus highlight the need for careful ML model deployment.

\begin{comment}
\begin{tiny}
\begin{verbatim}


1. An essential prerequisite of several attacks targeting machine learning algorithms
is knowing the architecture of the oracle model.

- All these attacks assume no access to the training data.
- A common step in model extraction attacks, model inversion attacks and membership inference
attacks is to retrain a substitute/shadow network using synthetic data sets.
- An implicit prerequisite is to train the substitute network using the same architecture 
as the oracle one.

1) model extraction attacks
For neural networks, it uses retraining techniques to train a substitute network using 
the same architecture.



2) membership inference attacks and model inversion attacks.
Both attacks try to analyze the relationship between a model and its training data set.
- It is clearly stated in membership inference attacks paper that
"the shadow models must be trained in a similar way to the oracle model".
- For neural networks, it refers to using the same architecture of a network.


(TODO: If time permitted, ask Reza for code, and do experiments
to show the attack does not work if using different architectures.)



2. There is no practical approach to extract the architecture of a neural network.

(TODO: Machine learning algorithms include decision tree, SVM,
neural networks etc. We focus on neural network in this paper.)

We discuss possible approaches and their limitations.

1) Ateniese et al. assumes the oracle classifier can be extracted from the binary executable 
for the target machine learning task through, for instance, dynamic analysis techniques.
- Not effective if executable files are not available.


2) Shokri et al. proposes that the attacker can use exactly the same service (e.g., Google
Prediction API) to train the substitute model as was used to train the oracle model.
- Work for platforms which do not provide users flexibility to define 
the model structure, model parameters, or training meta-parameters.
- Not work for platforms, such as Microsoft Azure ML, which allow
user-defined neural networks in a fine grained style.
Specifically, in Microsoft Azure ML, users can decide number of layers, 
number of neurons in each layer, activation function etc.
- Not work for other user defined models which are not trained using MLaaS platforms.


3) Brute force search. 
(TODO: Need experiment results.)

Note: Should we compare our approach against brute force search in evaluation?

An attacker can brute force search all possible architectures to find the one
matches the oracle architecture.
- Assuming attackers know the range for hyper-parameters, therefore the search space is bounded.
- Assuming attackers adopts an uniform retraining approach to train substitute
networks using different architectures with a synthetic training data set.
- Expected result:
All models work similar on synthetic test set, but differently on oracle test set.
This is because the synthetic data set has different distribution from the oracle data set.
Therefore, brute force search can not help to find the correct architecture.
 
 
3. We did an experiment to show the importance of using the same architecture 
in model extraction attacks.

Assuming the attacker has no access to training data, does not know the architecture.
It uses active learning: explain what active learning is, adaptive retraining.
-> uniformly generate random training data
-> after each round, using jacobian augmentation to generate data close to decision boundary,
-> query the oracle model to get label for each data

We train an oracle model using a DNN with
- 2 fully-connected layer, 1 softmax layer
- 1024 neurons in each layer
- tanh as activaction function

We train the oracle model using "Human Activity Recognition Using Smartphones Data Set"
~\footnote{http://archive.ics.uci.edu/ml/datasets/Human+Activity+Recognition+Using+Smartphones}.

We train four substitute networks with varied architecutres,
- same number of neurons in each layer, same activaaction function,
- differ in number of fully-connected layers

We evaluate the substitute model using two matrices:
1) a uniformly generated random data set, which is accessible by attacker
2) training data and test data set from the benchmark, which conforms to actual distribution of data,
but not accessible to the attacker

table:
            accuracy using (1), accuracy using (2)
1-layer: 98.18%, 43.65%
2-layer: 98.77%, 94.92%
3-layer: 99.03%, 92.25%
4-layer: 99.22%, 89.33%


 
 

In this paper, we propose a practical approach to extract the architecture of a neural network
using cache-based side channel attacks.
Our attack results strengthen multiple other attacks by achieving their prerequisites,
and thus highlight the need for careful ML model deployment.


\end{verbatim}
\end{tiny}
\end{comment}
